HeSP: a simulation framework for solving the task scheduling-partitioning problem on heterogeneous architectures

In this paper we describe HeSP, a complete simulation framework to study a general task scheduling-partitioning problem on heterogeneous architectures, which treats recursive task partitioning and scheduling decisions on equal footing. Considering recursive partitioning as an additional degree of freedom, tasks can be dynamically partitioned or merged at runtime for each available processor type, exposing additional or reduced degrees of parallelism as needed. Our simulations reveal that, for a specific class of dense linear algebra algorithms taken as a driving example, simultaneous decisions on task scheduling and partitioning yield significant performance gains on two different heterogeneous platforms: a highly heterogeneous CPU-GPU system and a low-power asymmetric big.LITTLE ARM platform. The insights extracted from the framework can be further applied to actual runtime task schedulers in order to improve performance on current or future architectures and for different task-parallel codes.

==> abstract_sent.tex <==
Task-based programming models and runtime task schedulers have demonstrated their potential to efficiently exploit 
parallelism on homogeneous and heterogeneous platforms, and to asynchronously handle task parallelism with minimal
user intervention. 
%
However, as heterogeneity increases in modern architectures, optimal task scheduling and balanced resource usage can become
major challenges, especially when complex data dependences and irregular degrees of parallelism arise in applications.
%
%However, the increase of architectural complexity, usually translated into higher heterogeneity, exposes serious 
%burdens to achieve near-optimal performance while maintaining programmability, being the problem aggravated when 
%complex data dependences among tasks arise.
%
In this paper, we present HeSP, a complete framework to study a more general task scheduling/partitioning problem
on heterogeneous architectures, which treats recursive task partitioning and scheduling decisions on equal footing. 
Considering data partitioning as an aditional degree of freedom, tasks can be dynamically partitioned or merged at 
runtime for each available processor type, exposing additional or reduced degrees of parallelism as needed. 
%
Our simulations reveal that, for a specific class of dense linear algebra algorithms taken as a driving example, 
simultaneous decisions on task scheduling and partitioning yield significant performance gains 
on two different heterogeneous platforms: a highly heterogeneous CPU-GPU system and a low-power asymmetric 
big.LITTLE ARM platform.
% 
The insights extracted from the framework can be further applied to actual runtime task schedulers in order
to improve performance on current or future architectures and for different task-parallel codes.


==> s5-dynamic.tex <==
\section{Towards dynamic scheduling-partitioning}
SHORTEN THIS TODO!!!

At this point, we chose OmpSs as the central programming model in the following discussion, since we believe is one of the most promising arenas in which this scheduling-partitioning problems might be attacked from the dynamic perspective. The following facts about OmpSs were considered when trying to devise ways of porting this scheduling-partitioning approach towards a runtime perspective.
 
\begin{itemize}
\item General task-based programming model, not restricted to linear algebra.
\item Support for heterogeneous hardware --e.g. SMPs, GPUs, Xeon Phi, ARM bigLITTLE-- and several task implementations \cite{versioning}, supporting CUDA and OpenCL codes.
\item Support for a wide range of systems: distributed MPI, shared-memory systems and SoCs(?).
\item Based on OpenMP language, with a code-to-code compiler that parses \textit{pragmas}.
\item It motivated the OpenMP 4.0 task extension \cite{openmpweb}.
\item Offers quite reach behavior from scheduling perspective, providing several schedulers and caching policies.
\item Its modulable, from the developer perspective. The runtime behavior can be extended with additional runtime plugins.
\end{itemize}

In listing \ref{lst:pragma_part} is illustrated how the partitioners could be included at OmpSs compiler level. Analogously to their already implemented/functioning pragmas (\textit{pragma omp task} and \textit{implements}), is worth noting that there is no conceptual difference between them.

%\lstinputlisting[float=t,frame=lines,caption=C Example of common OmpSs task annotations (lines 1 to 7) and the OmpSs partitioner annotation proposal (line 9).,label=lst:pragma_part]{Codes/pragma_part.c}

At runtime level, the partitioner variables specified would be considered in the scheduler-partitioner behavior. How to make this behavior powerful is a challenge, and it would probably require its reinforcement with additional information --such as performance models--, and efficient and lightweight heuristics to properly anticipate partial schedules associated to a hypothetical partitioning decision. 

Finally, it is worth considering its runtime applicability exclusively to linear algebra applications, out of the OmpSs scope. Since partitioners are mere extensions of simple tiling algorithms, we believe that including partitioners into a unified heterogeneous BLAS-LAPACK framework (like MAGMA or so) could be quite feasible and in principle not so hard to implement.

Overall, it is obvious that this scheduling-partitioning approach requires a lot of research and critics in order to push it forward to a real time scheduling scenario. Specifically, future research concerning both constructive and iterative solvers might yield promising developments in order to have efficient constructive and constructive-iterative heuristics at runtime.
